Learning Stochastic Graph Neural Networks with Constrained Variance

Stochastic graph neural networks (SGNNs) are information processing architectures that learn representations from data over random graphs. SGNNs are trained with respect to the expected performance, which comes with no guarantee about deviations of particular output realizations around the optimal expectation. To overcome this issue, we propose a variance-constrained optimization problem for SGNNs, balancing the expected performance and the stochastic deviation. An alternating primal-dual learning procedure is undertaken that solves the problem by updating the SGNN parameters with gradient descent and the dual variable with gradient ascent. To characterize the explicit effect of the variance-constrained learning, we conduct a theoretical analysis on the variance of the SGNN output and identify a trade-off between the stochastic robustness and the discrimination power. We further analyze the duality gap of the variance-constrained optimization problem and the converging behavior of the primal-dual learning procedure. The former indicates the optimality loss induced by the dual transformation and the latter characterizes the limiting error of the iterative algorithm, both of which guarantee the performance of the variance-constrained learning. Through numerical simulations, we corroborate our theoretical findings and observe a strong expected performance with a controllable standard deviation.

==> Conclusion.tex <==
%!TEX root = mainOp.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Conclusions   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions} \label{sec:conclusion}

In this paper, we consider the optimal resource allocation in free space optical networks. The problem takes the form of constrained stochastic optimization, that is typically challenging due to the non-convex nature, multiple constraints and lack of model information. Examples include power adaptation, relay selection and their joint allocation. We first propose the model-based Stochastic Dual Gradient algorithm, which solves the problem exactly by exploiting a null duality gap property. However, it heavily relies on system models that may not be available in practice. The model-free Primal-Dual Deep Learning algorithm is then developed to overcome these issues. In particular, it parameterizes the resource allocation policy with Deep Neural Networks and learns optimal parameters by updating primal and dual variables simultaneously. Policy gradient method is further applied to the primal update in order to estimate necessary gradient information without using the knowledge of system or channel models. Numerical experiments are performed in a number of applications to show superior performance of our algorithms. The model-free PDDL algorithm proposed in this paper has wide applications for problems in FSO networks and communications, where optical systems  are too sophisticated and atmospheric channels are too complicated to model.

==> conclusions.tex <==
%!TEX root = mainStabilitySO3.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Conclusions   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> myTikzDefs.tex <==

% This is a global control on the scale of plots. The constant \myfactor can be defined inside of an individual picture. It is good practice to reset \myfactor to 1 after the end of the picture.
\def\myfactor{1.0}
\def\unit{\myfactor cm}


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\footnotesize},   % Write numbers in tiny font
              label style = {font=\footnotesize}, % Write axes labels in footnote size font
              title style = {font=\footnotesize},
            }

% Definition of a graph node without filled in color. 
% Controls the appearance of a node in a graph plot
\tikzstyle{empty node} = [ circle, 
                     draw = black,
                     text = black, 
                     minimum size = 0.8*\unit]


% Definition of a graph node. Controls the appearance of a node in a graph plot
\tikzstyle{node} = [ empty node, 
                     fill = blue!50,
                     draw = blue!50,
                     text = white]

\tikzstyle{blue node} = [ empty node, 
                         fill = blue!50,
                         draw = blue!50,
                         text = white]

\tikzstyle{red node} = [ empty node, 
                         fill = red!50,
                         draw = red!50,
                         text = white]

\tikzstyle{green node} = [ empty node, 
                         fill = mygreen!50,
                         draw = mygreen!50,
                         text = white]


\tikzstyle{black node} = [ empty node, 
                           fill = black!40,
                           draw = black!40,
                           text = white]

                         
% Definition of a graph signal dot value without filled in color.
% These are smaller than the nodes and do not allow for text.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{empty dot} = [ circle, 
                           draw = black,
                           inner sep = 0pt,
                           anchor = center,
                           minimum size = 0.4*\unit]


% Definition of a graph signal dot value.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{dot} = [ empty dot, 
                    fill = blue!50,
                    draw = blue!50]

\tikzstyle{blue dot} = [ empty dot, 
                         fill = blue!50,
                         draw = blue!50]

\tikzstyle{red dot} = [ empty dot, 
                        fill = red!50,
                        draw = red!50]

\tikzstyle{black dot} = [ empty dot, 
                          fill = black!50,
                          draw = black!50]


% Definition of graph edges. An edge is undirected and doesn't contain arrows. A directed edge has an arrow at the end and a double directed edge contains two arrows. The latter is to be used when we want to emphasize the double directivity.
\tikzstyle{edge}                 = [shorten >=1pt, shorten <=1pt]
\tikzstyle{directed edge}        = [edge, -stealth]
\tikzstyle{double directed edge} = [edge, stealth-stealth]
\tikzstyle{tight edge}                 = [shorten >=0pt, shorten <=0pt]


% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]


==> nn_mimo.tex <==
\def\layersep{3.7cm}


\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=.8*\layersep, scale=0.6, transform shape]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{tneuron}=[circle,line width=1.2pt,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!25];
    \tikzstyle{output neuron}=[neuron, fill=red!25];
    \tikzstyle{hidden neuron}=[tneuron, fill=blue!25];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
  %  \foreach \name / \y in {1,...,6}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left: $h_{1}$] (I-1) at (0,-1) {};
        \node[input neuron, pin=left: $h_{2}$] (I-2) at (0,-2) {};
        \node[input neuron, pin=left: $h_{3}$] (I-3) at (0,-3) {};
        
        \node[input neuron, pin=left:] (I-4) at (0,-5) {};
        \node[input neuron, pin=left:] (I-5) at (0,-6) {};
        \node[input neuron, pin=left:] (I-6) at (0,-7) {};
        
% Draw the hidden layer nodes
    \foreach \name / \y in {1,2,3,4,5,6,7,8}
        \path[yshift=0.3cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.3cm]
            node[hidden neuron] (H-\name) at (2*\layersep,-2 cm-\y cm) {};

    % Draw the output layer node
    	\node[output neuron,pin={[pin edge={->}]right:$x_L^1$}] (O1) at (3*\layersep,-1 cm) {};
	\node[output neuron,pin={[pin edge={->}]right:$x_L^2$}] (O2) at (3*\layersep,-2 cm) {};
	\node[output neuron,pin={[pin edge={->}]right:$x_L^3$}] (O3) at (3*\layersep,-3 cm) {};
	\node[output neuron,pin={[pin edge={->}]right:$x_L^4$}] (O4) at (3*\layersep,-4 cm) {};
	\node[output neuron,pin={[pin edge={->}]right:}] (O5) at (3*\layersep,-6 cm) {};
	\node[output neuron,pin={[pin edge={->}]right:}] (O6) at (3*\layersep,-7 cm) {};
	%\node[output neuron,pin={[pin edge={->}]right:$\sigma^i$}, right of=H-3] (O2) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,6}
        \foreach \dest in {1,...,8}
            \path (I-\source) edge (H1-\dest);
            
     \foreach \source in {1,...,8}
        \foreach \dest in {1,...,4}
            \path (H1-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,4}
        \path (H-\source) edge (O1);
        
     \foreach \source in {1,...,4}
        \path (H-\source) edge (O2);
        
            \foreach \source in {1,...,4}
        \path (H-\source) edge (O3);
        
     \foreach \source in {1,...,4}
        \path (H-\source) edge (O4);
        
            \foreach \source in {1,...,4}
        \path (H-\source) edge (O5);
        
     \foreach \source in {1,...,4}
        \path (H-\source) edge (O6);

    % Annotate the layers
  %  \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
  %  \node[annot,left of=hl] {Input layer};
   % \node[annot,right of=hl] {Output layer};
\end{tikzpicture}



% End of code

==> proofsmainOp1.tex <==



\section{Proof of Theorem 1} \label{Appendix:proofOfTheorem1}

We will need the following lemma in the proof.

\begin{lemma} \label{lemma1}
Consider the underlying graph $\bbS = \bbV \bbLambda \bbV^\top$ and the perturbated graph $\hat{\bbS}$ with $N$ nodes.  The relative perturbation $\bbE= \bbU \bf{\Theta}\bbU^\top \in \ccalR $ satisfies $d(\bbS, \hbS) \le \| \bbE \| \le \epsilon$. Consider the integral Lipschitz filter [cf. Definition 1 in full paper] with $F=1$ input feature, $G=1$ output feature and integral Lipschitz constant $C_L$. Then, the output difference between filters $\bbB(\bbX; \bbS, \ccalB)$ and $\bbB(\bbX; \hat{\bbS}, \ccalB)$ satisfies
 \begin{equation} \label{eqn:thm10}
    \| \bbB(\bbX; \bbS, \ccalB) - \bbB(\bbX; \hat{\bbS}, \ccalB)\| \le 2C_L(1 + \sigma \sqrt{N})\| \bbX \| \epsilon + \ccalO(\epsilon^2)
\end{equation}
where $\delta = (\| \bbU - \bbV \|+1)^2-1$ implies the eigenvector misalignment between $\bbS$ and $\bbE$.
\end{lemma} 
\begin{proof}
With $F=1$ input feature $\bbX \in \mathbb{R}^{N \times 1}$ and $G=1$ output feature $\bbB(\bbX; \bbS, \ccalB), \bbB(\bbX; \hat{\bbS}, \ccalB) \in \mathbb{R}^{N \times 1}$, the output difference can be represented by
 \begin{equation} \label{eqn:thm10}
    \| \bbB(\bbX; \bbS, \ccalB) - \bbB(\bbX; \hat{\bbS}, \ccalB)\| = \big\| \sum_{k=0}^K b^{11}_k \bbS^k \bbX - \sum_{k=0}^K b^{11}_k \hbS^k \bbX \big\|
\end{equation}
with filter parameters $\ccalB = \{ b^{11}_0,\ldots,b^{11}_K \}$. We then refer to Theorem 3 in \cite{Gama19-Stability} to complete the proof.
\end{proof}

\begin{proof}[Proof of Theorem 1]
The output difference between $\bbPsi(\bbX; \bbS, \ccalA, \ccalB)$ and $\bbPsi(\bbX; \hbS, \ccalA, \ccalB)$ can be divided into the wide part difference and the deep part difference
 \begin{align}\label{eqn:thm100}
&\|\bbPsi(\bbX;\! \bbS, \ccalA,\! \ccalB)\!-\!\bbPsi(\bbX; \!\hbS, \ccalA,\! \ccalB)\| \\
&\le\! \|\bbPhi(\bbX;\! \bbS,\! \ccalA)\!-\!\bbPhi(\bbX;\! \hbS,\! \ccalA)\| \!+\! \|\bbB(\bbX;\! \bbS,\! \ccalB) \!-\! \bbB(\bbX;\! \hat{\bbS},\! \ccalB)\| \nonumber
\end{align}
where the triangle inequality is used. Let us consider these two terms separately.

\textbf{The wide term.} By using Lemma \ref{lemma1}, we bound the wide part difference as 
 \begin{equation} \label{eqn:thm11}
    \| \bbB(\bbX; \bbS, \ccalB) - \bbB(\bbX; \hat{\bbS}, \ccalB)\| \le 2C_L(1 + \sigma \sqrt{N}) \epsilon + \ccalO(\epsilon^2)
\end{equation}
 
\textbf{The deep term.} At layer $\ell$, the graph convolution can be considered as the application of $F_{\ell-1}F_\ell$ filters, i.e.,
\begin{equation}\label{eqn:thm12} 
 \left[\sum_{k=0}^{K} \bbS^{k} \bbX_{\ell-1} \bbA_{\ell k}\right]_f = \sum_{g=1}^{F_{\ell-1}} \sum_{k=0}^K a_{\ell k}^{fg} \bbS^k [\bbX_{\ell-1}]_{g} 
\end{equation}
for $f=1,\ldots, F_\ell$, where $a_{\ell k}^{fg} = [\bbA_{\ell k}]_{fg}$ is the $(f,g)$th entry of matrix $\bbA_{\ell k}$ and $[\cdot]_f$ represents the $f$th column. We denote by $\bbG_\ell^{fg}(\bbS)[\bbX_{\ell-1}]_{g}= \sum_{k=0}^K a_k^{fg} \bbS^k [\bbX_{\ell-1}]_{g}$ and $\bbx^g_{\ell-1} = [\bbX_{\ell-1}]_{g}$ for convenience of following derivation. By using \eqref{eqn:thm12} and substituting the GNN architecture [(4) in full paper] into the deep part difference, we get
 \begin{align} \label{eqn:thm13}
&\|\bbPhi(\bbX;\! \bbS,\! \ccalA)\!-\!\bbPhi(\bbX;\! \hbS,\! \ccalA)\| \\
&= \big\| \sigma\big( \sum_{f=1}^{F_{L-1}} \bbG_L^{1f}(\bbS)\bbx^f_{L-1} \big) - \sigma\big( \sum_{f=1}^{F_{L-1}} \bbG_L^{1f}(\hbS)\hat{\bbx}^f_{L-1} \big) \big\| \nonumber\\
&\le \sum_{f=1}^{F_{L-1}}  \big\| \bbG_L^{1f}(\bbS)\bbx^f_{L-1} - \bbG_L^{1f}(\hbS)\hat{\bbx}^f_{L-1} \big\| \nonumber
\end{align}
where the second inequality is because the nonlinearity $\sigma$ is normalized Lipschitz and the triangle inequality. By adding and substracting $\bbG_L^{1f}(\hbS)\bbx^f_{L-1}$ into the terms in the norm, we have
 \begin{align} \label{eqn:thm14}
&\big\| \bbG_L^{1f}\!(\bbS)\bbx^f_{L\!-\!1} \!-\! \bbG_L^{1f}\!(\hbS)\hat{\bbx}^f_{L\!-\!1} \big\|\\ &\!\le\! \big\| \bbG_L^{1f}\!(\bbS)\bbx^f_{L\!-\!1} \!\!-\! \bbG_L^{1f}\!(\hbS)\bbx^f_{L\!-\!1} \!\big\| \!+\!\! \big\|\bbG_L^{1f}\!(\hbS)\bbx^f_{L\!-\!1} \!\!-\! \bbG_L^{1f}\!(\hbS)\hat{\bbx}^f_{L\!-\!1} \!\big\| \nonumber \\
& \le \!\big\| \bbG_L^{1f}\!(\bbS)\bbx^f_{L\!-\!1} \!-\! \bbG_L^{1f}\!(\hbS)\bbx^f_{L\!-\!1} \big\| \! +\! \| \bbG_L^{1f}\!(\hbS) \| \big\|\bbx^f_{L\!-\!1} \!-\! \hat{\bbx}^f_{L\!-\!1} \big\|\nonumber
\end{align}
For the first term in \eqref{eqn:thm14}, by using Lemma \ref{lemma1}, we get
\begin{align} \label{eqn:thm15}
&\big\| \bbG_L^{1f}\!(\bbS)\bbx^f_{L-1} - \bbG_L^{1f}(\hbS)\bbx^f_{L-1} \big\| \\
& \le 2C_L(1 + \sigma \sqrt{N}) \|\bbx^f_{L-1}\| \epsilon + \ccalO(\epsilon^2).\nonumber
\end{align}
In terms of the term $\|\bbx^f_{L\!-\!1}\|$, we observe that 
\begin{align} \label{eqn:thm16}
&\|\bbx^f_{L\!-\!1}\| = \big\| \sigma\big( \sum_{g=1}^{F_{L-2}} \bbG_{L-1}^{fg}(\bbS)\bbx^g_{L-2} \big) \big\| \\
&\le  \sum_{g=1}^{F_{L-2}} \big\| \bbG_{L-1}^{fg}(\bbS)\bbx^g_{L-2} \big\| \le \sum_{g=1}^{F_{L-2}} \big\| \bbx^g_{L-2} \big\|\nonumber
\end{align}
where we use the triangle inequality, followed by the bound on filters \cite{Ortega18-GSP}, i.e., the filter frequency response $|a^{fg}_{L-1}(\lambda)| = \big| \sum_{k=0}^K a_{(L-1)k}^{fg} \lambda^k \big| \le 1$. We follow this recursion to obtain
\begin{equation} \label{eqn:thm17}
\|\bbx^f_{L\!-\!1}\| \le \prod_{\ell = 1}^{L-2} F_\ell \big\| \bbx^1_0 \big\|
\end{equation}
where $\| \bbx^1_0 \| = \| \bbX \|$ by definition since the number of input feature $F_0=F=1$. By substituting \eqref{eqn:thm17} into \eqref{eqn:thm15}, we have
\begin{align} \label{eqn:thm18}
&\big\| \bbG_L^{1f}\!(\bbS)\bbx^f_{L-1} - \bbG_L^{1f}\!(\hbS)\bbx^f_{L-1} \big\| \\
&\le  2C_L(1 + \sigma \sqrt{N})\prod_{\ell = 1}^{L-2} F_\ell \big\| \bbX \big\| \epsilon + \ccalO(\epsilon^2). \nonumber
\end{align}
For the second term in \eqref{eqn:thm14}, by again using the filter bound \cite{Ortega18-GSP}, we get
\begin{equation} \label{eqn:thm19}
\| \bbG_L^{1f}\!(\hbS) \| \big\|\bbx^f_{L\!-\!1} \!-\! \hat{\bbx}^f_{L\!-\!1} \big\| \le \big\|\bbx^f_{L\!-\!1} \!-\! \hat{\bbx}^f_{L\!-\!1} \big\|.
\end{equation}
By substituting \eqref{eqn:thm18} and \eqref{eqn:thm19} into \eqref{eqn:thm14} and the latter into \eqref{eqn:thm13}, we have
 \begin{align} \label{eqn:thm110}
&\|\bbPhi(\bbX;\! \bbS,\! \ccalA)\!-\!\bbPhi(\bbX;\! \hbS,\! \ccalA)\| \\
&\le\! \sum_{f=1}^{F_{L-1}}\!\big\|\bbx^f_{L\!-\!1} \!-\! \hat{\bbx}^f_{L\!-\!1} \big\| \!+\! 2C_L(1 \!+\! \sigma \sqrt{N})\!\prod_{\ell = 1}^{L-1} F_\ell \big\| \bbX \big\| \epsilon \!+\! \ccalO^2(\epsilon).\nonumber
\end{align}
From \eqref{eqn:thm110}, we observe that the output difference of $L$th layer depends on that of $(L-1)$th layer. Repeating this recursion until the input layer, we have
 \begin{align} \label{eqn:thm111}
&\|\bbPhi(\bbX; \bbS, \ccalA)-\bbPhi(\bbX; \hbS, \ccalA)\| \\
&\le 2C_L(1 + \sigma \sqrt{N}) L \prod_{\ell = 1}^{L-1} F_\ell \big\| \bbX \big\| \epsilon + \ccalO^2(\epsilon) \nonumber
\end{align}
where we use the initial condition $\| \bbx_0^1 - \hat{\bbx}_0^1 \| = \| \bbX - \bbX \|=0$.

Together, by substituting \eqref{eqn:thm11} and \eqref{eqn:thm111} into \eqref{eqn:thm100}, we complete the proof
 \begin{align}\label{eqn:thm112}
&\|\bbPsi(\bbX;\! \bbS, \ccalA,\! \ccalB)\!-\!\bbPsi(\bbX; \!\hbS, \ccalA,\! \ccalB)\| \\
&\le\! 2C_L(1 + \sigma \sqrt{N}) \left(\! |\alpha_W| \!+\! |\alpha_D| L \prod_{\ell = 1}^{L-1} F_\ell \!\right)\! \big\| \bbX \big\| \epsilon \!+\! \ccalO^2(\epsilon).\nonumber
\end{align}

\end{proof}



\section{Proof of Theorem 2} \label{Appendix:proofOfTheorem2}

\begin{proof}

Let $\ccalA^{\dag}$ and $\ccalB^{\dag}$ be the parameters learned from the offline training phase. The proposed online learning procedure fixes the deep part, i.e., it freezes the parameters $\ccalA = \ccalA^{\dag}$, and retrains the wide part online. The model $\bbPsi(\bbX; \bbS, \ccalA, \ccalB)$ can then be represented as a function of the wide part parameters $\ccalB$ only
 \begin{align}\label{proof:theorem1eq1}
\bbPsi(\bbX; \bbS, \ccalA^{\dag}, \ccalB) &= \alpha_{\text{D}} \bbPhi(\bbX; \bbS, \ccalA^{\dag}) + \alpha_{\text{W}} \bbB(\bbX; \bbS, \ccalB) + \beta \nonumber\\
& = \hat{\bbPsi}(\bbX; \bbS, \ccalB).
\end{align}
Given the graph signal $\bbX$ and the graph matrix $\bbS$, $\hat{\bbPsi}(\bbX; \bbS, \ccalB)$ is a linear function of $\ccalB$ since both the graph filter $\bbB(\bbX; \bbS, \ccalB)$ and the combination way of two components are linear.

At testing time $t$, the sampled optimization problem \eqref{eq:timevaryingp} is translated to
 \begin{equation}\label{eq:timevaryingp1}
\min_{\ccalB} J_t\big(\hat{\bbPsi}(\bbX_t; \bbS_t, \ccalB)\big)
\end{equation}
where $J_t(\cdot)$, $\bbX_t$ and $\bbS_t$ are given instantaneous loss function, observed signal and graph matrix at time instance $t$. Since $\hat{\bbPsi}(\bbX_t; \bbS_t, \ccalB)$ is a linear function of $\ccalB$, $J_t\big(\hat{\bbPsi}(\bbX_t; \bbS_t, \ccalB)\big)$ is differentiable, strongly smooth with constant $C_{t,s}$ and strongly convex with constant $C_{t,\ell}$ based on Assumption 2.

We then formally prove the convergence of the online learning procedure and denote by $J_t(\ccalB)=J_t\big(\bbPsi(\bbX_t; \bbS_t, \ccalA^{\dag}, \ccalB)\big)$ as the concise notation for convenience of derivation. From the online learning iteration, we have
 \begin{equation}\label{proof:theoremm21}
\ccalB_{t+1} = \ccalB_{t}-\gamma \nabla_{\ccalB} J_t\big(\ccalB_t\big).
\end{equation}
Subtracting $\ccalB_{t}^*$ in both sides of \eqref{proof:theoremm21} yields
 \begin{align}\label{proof:theoremm22}
&\|\ccalB_{t+1} - \ccalB_t^*\|^2 = \|\ccalB_{t}-\ccalB_t^* - \gamma \nabla_{\ccalB} J_t( \ccalB_t )\|^2.
\end{align}
Further since $\nabla_{\ccalB} J_t( \ccalB_t^* ) = 0$ due to the optimality of convex problems, we can get
 \begin{align}\label{proof:theoremm23}
&\|\ccalB_{t+1} \!-\! \ccalB_t^*\| \!=\! \|\big(\ccalB_{t} \!-\! \gamma \nabla_{\ccalB} J_t( \ccalB_t )\big) \!-\! \big(\ccalB_t^* \!-\! \nabla_{\ccalB} J_t( \ccalB_t^* ) \|. 
\end{align}
We now consider the operator $f(\ccalB) = \ccalB - \gamma \nabla_{\ccalB} J_t( \ccalB )$. If $J_t( \ccalB )$ is strongly smooth with constant $C_{t,s}$ and strongly convex with constant $C_{t,\ell}$, $f(\ccalB)$ is a contraction operator with the contraction factor $m_t = \max \{ |1-\sigma C_{t,s}|, |1-\sigma C_{t,\ell}| \}$ \cite{}, i.e., we have
 \begin{align}\label{proof:theoremm24}
\|f(\ccalB_t) \!-\! f(\ccalB^*_t)\| &\!=\! \|\big(\ccalB_{t} - \gamma \nabla_{\ccalB} J_t( \ccalB_t )\big) - \big(\ccalB_t^* - \nabla_{\ccalB} J_t( \ccalB_t^* ) \| \nonumber \\
& \le m_t \|\ccalB_t - \ccalB_t^* \|.
\end{align}
By substituting \eqref{proof:theoremm24} into \eqref{proof:theoremm23} and adding and subtracting $\ccalB_{t+1}^*$, we have
 \begin{align}\label{proof:theoremm25}
&\|\ccalB_{t+1} - \ccalB_{t+1}^* + \ccalB_{t+1}^* - \ccalB_t^*\| \\
& \le \|\ccalB_{t+1} - \ccalB_{t+1}^*\| + \|\ccalB_{t+1}^* - \ccalB_t^*\| \nonumber\\
&\le m_t \|\ccalB_t - \ccalB_t^* \| + \|\ccalB_{t+1}^* - \ccalB_t^*\|.\nonumber 
\end{align}
By using the fact $\|\ccalB_{t+1}^* - \ccalB_t^*\| \le C_B$ from Assumption \ref{asm:1}, we get
 \begin{align}\label{proof:theoremm26}
&\|\ccalB_{t+1} - \ccalB_{t+1}^* + \ccalB_{t+1}^* - \ccalB_t^*\| \le m_t \|\ccalB_t - \ccalB_t^* \| + C_B.
\end{align}
Unrolling this process to the initial condition completes the proof
 \begin{equation}\label{eq:H}
\| \ccalB_t - \ccalB_t^* \| \le \big( \prod_{\tau=1}^t m_{\tau} \big) \| \ccalB_0 - \ccalB_0^* \| + \frac{1-\hat{m}^{t}}{1-\hat{m}} C_B
\end{equation}
where $m_t=\max\{ |1-\gamma C_{t,s}|, |1-\gamma C_{t,\ell}| \}$ is the convergence rate and $\hat{m}= \max_{1 \le \tau \le t} m_\tau$.
\end{proof}



\section{Proof of Proposition 1} \label{Appendix:proofOfProposition1}


\begin{proof}
By adding and subtracting $\gamma/n \sum_{i=1}^n \bbg_{i,k}$ in both sides of \eqref{eq:disgdMatrixStopRecursiveNode}, we have
\begin{align}\label{proof:prop11}
&\|\ccalC(k+1) - \ccalB^*_{k+1}\| \\
&= \big\| \ccalC(k) \!-\! \ccalB^*_{k+1} - \frac{\gamma}{N} \sum_{i=1}^N \bbg_{i,k} +\frac{\gamma}{N} \sum_{i=1}^N \bbg_{ij,k} - \frac{\gamma}{N} \sum_{i=1}^N \bbd_{i,k}\big\| \nonumber\\
&\le\! \big\| \ccalC(k) - \ccalB^*_{k+1} \!-\! \frac{\gamma}{N} \sum_{i=1}^N \bbg_{i,k}\big\| \!+\!\big\|\frac{\gamma}{N} \sum_{j=1}^N \bbg_{i,k} \!-\! \frac{\gamma}{N} \sum_{i=1}^N \bbd_{i,k}\big\| \nonumber
\end{align}
where the triangle inequality is used. We consider two terms in the bound of \eqref{proof:prop11} separately. For the first term $\big\| \ccalC(k) - \ccalB^*_{k+1} \!-\! \gamma/N \sum_{i=1}^N \bbg_{i,k}\big\|$ in \eqref{proof:prop11}, note that $\ccalC(k) - \gamma/N \sum_{i=1}^N \bbg_{i,k}$ is a gradient descent iteration of $1/N\sum_{i=1}^N J_{i,k}\big(\bbPsi(\bbX_k; \bbS_k, \ccalA^{\dag}, \ccalB)\big)$ at the decision variable $\ccalC(k)$ with the step-size $\gamma$. From the result of Theorem \ref{thm:convergence}, we know that
\begin{align}\label{proof:prop12}
&\big\| \ccalC(k) \!-\! \frac{\gamma}{N} \sum_{i=1}^N \bbg_{i,k} \!-\! \ccalB^*_{k+1} \big\| \!\le\! m_k \|\ccalC(k) \!-\! \ccalB^*_k\| \!+\! C_B
\end{align}
where $m_k = \max\{ |1-\gamma C_{t,s}|,|1-\gamma C_{t,\ell}| \}$ is the convergence rate. For the second term $\|\gamma/N \sum_{i=1}^N \bbg_{i,k} - \gamma/N \sum_{i=1}^N \bbd_{i,k}\|$, we can bound it with the triangular inequality as
\begin{equation}
\begin{aligned}\label{proof:prop13}
&\|\frac{\gamma}{N} \sum_{i=1}^N \bbg_{i,k} - \frac{\gamma}{N} \sum_{i=1}^N \bbd_{i,k}\| \le \frac{\gamma}{N} \sum_{i=1}^N \|  \bbg_{i,k} -  \bbd_{i,k}\|.
\end{aligned}
\end{equation}
From the strongly convexity in Assumption \ref{asm:2}, we have
\begin{equation}
\begin{aligned}\label{proof:prop14}
& \|  \bbg_{i,k} -  \bbd_{i,k}\| \le C_{k,\ell} \| \ccalC(k) - \ccalB_{i,k} \|.
\end{aligned}
\end{equation}
By substituting \eqref{proof:prop14} into \eqref{proof:prop13} and altogether into \eqref{proof:prop11} with \eqref{proof:prop12}, we get
\begin{equation}
\begin{aligned}\label{proof:prop15}
&\|\ccalC(k+1) - \ccalB^*_{k+1}\| \\
& \le m_k \|\ccalC(k) - \ccalB^*_k\| + \frac{\gamma C_{k,\ell}}{N} \sum_{i=1}^n \| \ccalC(k) - \ccalB_{i,k} \| + C_B
\end{aligned}
\end{equation}
completing the proof.
\end{proof}

\section{Proof of Theorem 3}\label{Appendix:proofOfTheorem3}

\begin{proof}

From \eqref{eq:disgdMatrixStopRecursiveNode}, we know that
\begin{equation}
\begin{aligned}\label{proof:thm31}
\ccalC(k) = \ccalC(0) - \frac{\gamma}{N}\sum_{\kappa = 0}^{k-1} \sum_{i=1}^N \bbd_{i,\kappa}
\end{aligned}
\end{equation}
for all $k \ge 1$ with $\ccalC(0)=1/N \sum_{i=1}^N \ccalB_{i,0}$. By comparing \eqref{proof:thm31} with the distributed online update in \eqref{eq:disgd}, we have
\begin{align}\label{proof:thm32}
&\|\ccalC(k) - \ccalB_{i,k}\| \le \Big\| \sum_{j=1}^N \big( \frac{1}{N} - [\bbLambda(0,k-1)]_{j}^i \big) \ccalB_{j,0} \\
& \!-\!\gamma\! \sum_{\kappa =1}^{k-1}\! \sum_{j\!=\!1}^N\!\! \big(\! \frac{1}{N} \!\!-\! [\bbLambda(0,\!k\!-\!\!1)]_{j}^i \big) \bbd_{j,\kappa\!-\!1} \!-\! \gamma \big( \frac{1}{N}\!\! \sum_{j=1}^N\! \bbd_{j,k\!-\!1} \!-\! \bbd_{i,k\!-\!1} \!\big)\!\Big\|\nonumber
\end{align}
where $\bbLambda(0,k-1) = \prod_{t = 0}^{k-1}\bbW_{t}$ is the production of a sequence of weight matrices. By using the triangle inequality, we can bound \eqref{proof:thm32} as
\begin{align}\label{proof:thm33}
\|\ccalC(k) - \ccalB_{i,k}\| \!&\le\! \max_{1 \le j \le N}\| \ccalB_{j,0} \| \sum_{j=1}^N \big| \frac{1}{N} \!-\! [\bbLambda(0,k\!-\!1)]_{j}^i \big|  \\
& +\gamma \sum_{\kappa =1}^{k-1} \sum_{j=1}^N \| \bbd_{j,\kappa-1} \| \big| \frac{1}{N} - [\bbLambda(0,k-1)]_{j}^i \big|  \nonumber \\
&-\frac{\gamma}{N} \sum_{j=1}^N \Big\| \bbd_{j,k-1} - \bbd_{i,k-1} \Big\|\nonumber.
\end{align}
By using the result of Lemma \ref{lemma:limitMatrix} in the first two terms of \eqref{proof:thm33}, the result of Proposition \ref{Prop:iterationRelation} in the third term of \eqref{proof:thm33} and the assumptions $\| \ccalB_{j,0} \| \le C_{0,\ell}$ and $\| \bbd_{i,k} \| \le C_{k,\ell}$, we get 
\begin{equation}
\begin{aligned}\label{proof:thm34}
&\|\ccalC(k) - \ccalB_{i,k}\| \\
& \le 2 \gamma C_\ell \left( 1 + \frac{N}{1-(1-\epsilon^{B})^{1/B}} \frac{1+\epsilon^{-B}}{1-\epsilon^{B}} \right)
\end{aligned}
\end{equation}
with $C_\ell = \max_{1\le t \le k-1} C_{t,\ell}$. By substituting \eqref{proof:thm34} into the result of Proposition \ref{Prop:iterationRelation}, we have
\begin{equation}
\begin{aligned}\label{proof:thm35}
&\|\ccalC(k+1) - \ccalB^*_{k+1}\| \le m_k \|\ccalY(k) - \ccalB^*_k\| \!+\!2 \gamma^2 C_\ell^2 C_1 + C_B
\end{aligned}
\end{equation}
where 
\begin{equation}
\begin{aligned}\label{proof:thm36}
C_1 = 1 + \frac{N}{1-(1-\epsilon^{B})^{1/B}} \frac{1+\epsilon^{-B}}{1-\epsilon^{B}}
\end{aligned}
\end{equation}
is the concise notation. Unrolling this recursion, we obtain
\begin{equation}
\begin{aligned}\label{proof:thm37}
&\|\ccalC(k+1) - \ccalB^*_{k+1}\| \\
& \le \prod_{i=1}^k m_i \|\ccalC(0) - \ccalB^*_0\| \!+\!\frac{1-\hat{m}^k}{1-\hat{m}}\big( 2 \gamma^2 L^2 C_1 + C_B \big)
\end{aligned}
\end{equation}
where $\hat{m} = \max_{1\le t \le k} m_t$. Again using \eqref{proof:thm34} in \eqref{proof:thm37}, we complete the proof
\begin{equation}
\begin{aligned}\label{proof:thm38}
&\|\ccalB_{i,k+1} - \ccalB^*_{k+1}\| \\
& \le \prod_{i=1}^k m_i \|\ccalC(0) - \ccalB^*_0\| \!+\!\frac{2 \gamma^2 L^2 C_1 + C_B}{1-m} + 2 \gamma L C_1.
\end{aligned}
\end{equation}

\end{proof}






































